OpenSight: A Simple Open-Vocabulary Framework for LiDAR-Based Object Detection

Traditional LiDAR-based object detection research primarily focuses on closed-set scenarios, which falls short in complex real-world applications. Directly transferring existing 2D open-vocabulary models with some known LiDAR classes for open-vocabulary ability, however, tends to suffer from over-fitting problems: The obtained model will detect the known objects, even presented with a novel category. In this paper, we propose OpenSight, a more advanced 2D-3D modeling framework for LiDAR-based open-vocabulary detection. OpenSight utilizes 2D-3D geometric priors for the initial discernment and localization of generic objects, followed by a more specific semantic interpretation of the detected objects. The process begins by generating 2D boxes for generic objects from the accompanying camera images of LiDAR. These 2D boxes, together with LiDAR points, are then lifted back into the LiDAR space to estimate corresponding 3D boxes. For better generic object perception, our framework integrates both temporal and spatial-aware constraints. Temporal awareness correlates the predicted 3D boxes across consecutive timestamps, recalibrating the missed or inaccurate boxes. The spatial awareness randomly places some ``precisely'' estimated 3D boxes at varying distances, increasing the visibility of generic objects. To interpret the specific semantics of detected objects, we develop a cross-modal alignment and fusion module to first align 3D features with 2D image embeddings and then fuse the aligned 3D-2D features for semantic decoding. Our experiments indicate that our method establishes state-of-the-art open-vocabulary performance on widely used 3D detection benchmarks and effectively identifies objects for new categories of interest.

==> sec/0_abstract.tex <==

%Specifically, we feed the accompanying camera images of LiDAR data into the detection model to generate 2D boxes for generic objects.

% framework aiming to detect 3D bounding boxes for novel categories of interest.
%The fundamental challenge for open-set detection in LiDAR space lies in the limited availability of annotated training data in existing datasets, hindering the direct acquisition of diverse concepts.

%Besides the 3D ground truth supervision of known classes, we use the generated 2D boxes to supervise the objects in novel classes, preventing over-fitting on known categories.

% eliminates the necessity of known classes.

==> sec/3_method.tex <==
\section{OpenSight: Open-Vocabulary LiDAR-based Object Detection}
To elaborate on the LiDAR-based open-vocabulary object detection, we first briefly introduce the necessary notations for ease of understanding. Following this, we delve into the details of generic object perception in Section~\ref{subsection: generic object perception}. Subsequently, we present the process of specific semantic interpretation in Section~\ref{subsection: specific semantics interpretation}. The overall framework of OpenSight is presented in Figure~\ref{fig: overall framework.}.

% As our fundamental contribution is the pioneering introduction of
% in the context of autonomous driving
% and elaborate on the introduced temporal and spatial constraints
% and provide the precise label of a generic object

\subsection{Notation and Preliminaries}
The LiDAR dataset is denoted as $\mathcal{D} = \{P_i, \{y_k \}_{k=1}^K\}_{j=1}^{|\mathcal{D}|}$, where $P_i$ corresponds to the LiDAR point clouds in $i$-th frame, basically composed of $(x_i, y_i, z_i)$ coordinates. $y_k$ represents the combination of each 3D bounding box $b_k$ and its semantic label $c_k$. In open-vocabulary scenarios, $P_i$ is visible while $y_k$ is not. Generally, in the context of autonomous driving, each LiDAR frame is accompanied by $m$ images captured from varying perspectives. We define the image dataset as $\mathcal{I} = \{(I_{ij})_{j=1}^m\}_{i=1}^{|\mathcal{D}|}$ here. Image $I_{ij}$ in $j$-th view and LiDAR points $P_i$ could be connected by the intrinsic matrix $\textbf{K}_j$ and extrinsic matrix $\textbf{E}_j$. For clarity and brevity in the rest of the paper, we utilize a single LiDAR frame as an example and abbreviate and $I_{ij}$ as $I_j$, respectively. $N$ denotes the number of 3D objects, with $f^{3D}$ and $f^{2D}$ denotes the extracted feature in 3D and 2D space.

 %$Y_{3D}$ and  %$Y_i^{3D}$ 
% |\mathcal{D}|$ indicates the total number of frames within the dataset. 

%In a closed-set detection, $c_k \in R^C$ is spanned in space $R^C$ with $C$ as the number of categories considered. 
\subsection{Generic Objects Perception}
\label{subsection: generic object perception}
Discerning and localizing generic objects are fundamental in LiDAR-based open-vocabulary detection when ground-truth boxes and labels are absent. The model is expected to perceive the existence of a generic object before assigning specific labels.
This section details how we leverage 2D and 3D geometry priors to enable this perception, including initial box estimation, and temporal-spatial awareness. 
% We further structure this process into three distinct phases for clarity.

\noindent{\textbf{Initial Box Estimation.}} In practical applications, each LiDAR frame is typically paired with $m$ images $\{I_j\}_{j=1}^{m}$, captured from various perspectives. Each image is processed through the pre-trained detection model $\mathcal{I}$, yielding a set of 2D bounding boxes $\{b_{jk}\}_{k=1}^{V_j}$, where $V_j$ represents the number of 2D objects identified in the $j$-th viewpoint. By integrating the data from all viewpoints, we compile the collective set of detected boxes $\{(b_{jk}^{2D})_{k=1}^{V_j}\}_{j=1}^{m}$.

With the obtained 2D boxes of generic objects, we try to lift them back in the LiDAR space. Specifically, we project the LiDAR point $P_i$ into each image view by:
\begin{equation}
    \hat{P}_{ij} = \textbf{K}_j \cdot \textbf{E}_j \cdot P_i, \  j=1,...,m
\end{equation}
where $\textbf{E}_j$ and $\textbf{K}_j$ are extrinsic and intrinsic matrix, respectively. The points whose projection falls within each of the predicted 2D bounding boxes $b_{jk}^{2D}$ essentially constitute the 3D frustum, a conical region perceivable from a given perspective. We then apply the region growing algorithm~\cite{adams1994seeded} to isolate the cluster with the densest LiDAR points.

To estimate 3D bounding boxes from LiDAR point clusters, we first determine the extremal points along each axis by calculating the minimum and maximum coordinates. Take the X-axis for example, this is achieved by performing $x_{\min} = \min(\{x_i\}_{i=0}^{|N_c|})$ and $
x_{\max} = \max(\{x_i\}_{i=0}^{|N_c|})$.
These extremal points, identified similarly for the Y and Z axis, define the vertices of the bounding box. From these vertices, we construct the maximal bounding box $b_i^{3D}$, enclosing all points in the cluster. The 3D boxes for generic objects at timestamp $t$ are then finalized as $\mathcal{B}^t = \{b_{i}^{3D}\}_{i=0}^{N_t}$, by aggregating all boxes from $m$ perspectives.
%These extremal values define the vertices of the bounding box. Using these vertices, we derive the maximal bounding box $b_i^{3D}$ that encompasses all points in the cluster. We finalize the 3D boxes for generic objects at timestamp $t$ as $\mathcal{B}^t = \{b_{k}^{3D}\}_{k=1}^{V}$ by considering all $V$ 2D boxes across all $m$ perspectives.

% we consider a single cluster as an example. Suppose that the coordinates of the clustered LiDAR points are ${x_i, y_i, z_i}{i=0}^{|N_c|}$, where $|N_c|$ denotes the number of points in the cluster.


% due to its convenience. It inherently provides 2D bounding boxes, object features, and text embeddings in one operation.
%In our approach, we employ the ground DINO detection model for box extraction and curate the textual prompt $\mathcal{T}$ by a list of objects commonly encountered in autonomous driving. As long as these prompts are sufficiently comprehensive, they can encompass all generic objects within a single image. The formulated prompts $\mathcal{T}$, along with the 2D images $\mathcal{I}$, are input into the text and visual encoders, respectively, resulting in a set of 2D boxes $\{(b_{jk}^{2D})_{k=1}^{V_j}\}_{j=1}^{m}$.
% \begin{equation}
%     \{(b_{jk}^{2D})_{k=1}^{V_j}\}_{j=1}^{m} = f_{\rm grounding\ DINO}(\mathcal{T}, \mathcal{I})
% \end{equation}
%Only the predicted 2D boxes are used here and we do not focus on the semantic labels of generated boxes since our primary goal is to use these boxes to identify the existence of objects in novel classes. The 2D object features and text embeddings will be utilized for interpreting specific semantics in Section~\ref{subsection: specific semantics interpretation}. It is noteworthy that any detection model capable of providing object locations could be substituted for the one currently employed.

\begin{figure}[t]
  \centering
      \includegraphics[width=0.45\textwidth]{images/temporal.png}
  %\fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \vspace{-1em}
  \caption{Temporal awareness: Project boxes from frame $t+1$ to $t$. By comparing with projections, we refine predicted boxes in frame $t$ for missed or inaccurately estimated objects.}
  \label{fig: temporal.}
  \vspace{-2em}
\end{figure}
Considering that the majority of objects are lying on the ground and the occluded objects from one perspective, we adopt two filtering strategies to improve frustum construction. Firstly, to mitigate the impact of ground points on LiDAR point projection and clustering, we use RANSAC~\cite{fischler1981random} for ground plane estimation and exclude these points. 
Secondly, to remove the distortion from bounding box corners, largely caused by other overlapped objects, we apply the SAM method~\cite{kirillov2023segany}. By inputting the detected 2D boxes as prompts, we can obtain more accurate object contours.

%Then, we try to get a tighter contour of the objects to exclude the corner regions of bounding boxes, which introduces more distortion when the objects are overlapped. We use the detected 2D boxes as prompts and apply the latest SAM~\cite{} to achieve this. 

\noindent \textbf{Temporal Awareness.}
For the LiDAR point cloud, point density decreases sharply as distance increases, leading to less reliable estimations for distant objects. However, in autonomous driving scenarios, objects that are distant in the current frame may move closer in subsequent frames. To exploit this, we leverage the temporal continuity between frames by correlating 3D bounding box predictions across successive timestamps. We take frames at timestamp $t$ and $t+1$ as an example. Specifically, given the predicted boxes $\mathcal{B}^t = \{b_i\}_{i=0}^{N_t}$ and $\mathcal{B}^{t+1} = \{{b_i\}_{i=0}^{N_{t+1}}}$, where $N_{t+1}$ and $N_t$ represent the number of boxes in $t+1$ and $t$, respectively, we project each 3D box $b_i$ in $\mathcal{B}^{t+1}$ back to frame $t$ using the transformation:
\begin{equation*}
\hat{b}_i
= \textbf{E}_{\text{lidar} \leftarrow \text{ego}_{t}} \cdot
\textbf{E}_{\text{ego}_{t} \leftarrow \text{glb}} \cdot
\textbf{E}_{\text{glb} \leftarrow \text{ego}_{t+1}} \cdot
\textbf{E}_{\text{ego}_{t+1} \leftarrow \text{lidar}} \cdot
b_i,
\end{equation*}
where $\textbf{E}_{\text{lidar} \leftarrow \text{ego}_{t}}$ and 
$\textbf{E}_{\text{ego}_{t} \leftarrow \text{glb}}$ are the extrinsic matrices for the ego to LiDAR and global to ego transformations at timestamp $t$, and $\textbf{E}_{\text{glb} \leftarrow \text{ego}_{t+1}}$,
$\textbf{E}_{\text{ego}_{t+1} \leftarrow \text{lidar}}$ denotes ego to global and LiDAR to ego at timestamp $t+1$, respectively.

With all boxes in $\mathcal{B}^{t+1}$ considered, we obtain their projections as $\hat{\mathcal{B}}^{t+1}$ and construct the overlap matrix $M \in \mathbb{R}^{N_{t+1}\times N_t}$ by calculating their Intersection over Union (IoU) with boxes in $\mathcal{B}^{t}$. We address two key scenarios: If a box $\hat{b}_i$ has no overlap with boxes in $\mathcal{B}^{t}$, its counterpart $b_i$ in timestamp $t+1$ is considered a missed detection in the current frame and is added to the prediction at timestamp $t$. Conversely, if box $\hat{b}_i$ overlaps with boxes in $\mathcal{B}^{t}$ and its distance exceeds a certain threshold, we perform Non-Maximum Suppression (NMS) and retain the union of the two boxes to address potentially incomplete estimations at greater distances (See Figure~\ref{fig: temporal.}). 

This process updates the predicted boxes of the current frame to $\mathcal{B}^t_{\rm update} = \mathcal{B}^t \bigcup \mathcal{B}^t_{\rm temporal}$, which combines the original and temporally adjusted boxes. In practice, for the current frame, we consider both its subsequent frame at timestamp $t+1$ and its precedent frame at timestamp $t-1$. Through such a constraint, we are likely to boost the continuity and consistency of generic objects over time.

%Different from the operation in 3D space, we have $m$ views here. For each view, we perform bipartite matching. The cost is Based on this, we perform the Hungarian matching to get the label assignment on 2D space in each view, 

%The core idea above is trying to uncover as many as possible 3D boxes for novel objects.
\begin{figure}[t]
  \centering
      \includegraphics[width=0.48\textwidth]{images/spatial.png}
      % \fbox{\rule[0.5cm]{0cm}{2cm} \rule[-.5cm]{3cm}{0cm}}
  \vspace{-2em}
  \caption{Spatial awareness: Size priors are first generated from GPT-4 to select ``precisely'' estimated boxes and build the object bank. Randomly select objects and points from the objects bank and place them in the current frame $t$.}
  \label{fig: spatial.}
  \vspace{-2em}
\end{figure}
\noindent \textbf{Spatial Awareness.}
Considering the sparse object distribution in 3D LiDAR scans, where vast areas of the point cloud are often devoid of meaningful objects, we also focus on the systematic integration of ``precisely'' estimated objects in each frame to enhance the detectability and representation of generic objects.
% maintaining precisely estimated boxes an
To obtain these precise boxes from $\mathcal{B}^t$ in the absence of any ground truth, we utilize large language models (LLMs), such as GPT-4, for extracting useful size priors of objects. GPT-4, when prompted appropriately, can provide valuable insights into the typical sizes of objects within a specific class, \emph{e.g.}, the width, length, and height of a class. For instance, prompts like ``What is the average size of a \{\#CLASS\} in the autonomous driving scene?'' enable us to collect size statistics for common classes~(Details in the Appendix). Moreover, leveraging the ability of GPT-4 to process images, we also input images of the relevant objects to validate these size priors (See Figure~\ref{fig: spatial.}).

Utilizing the extracted size priors, we selectively retain 3D boxes in $\mathcal{B}^t$ that closely align with these priors. A box is reserved if its dimensions $w$, $l$, and $h$ fall within the specified range:
\begin{equation}
\label{equ: select box}
\begin{aligned}
    w &\in [(1-\tau)w_{prior}, (1+\tau)w_{prior}], \\
    \ell &\in [(1-\tau)\ell_{prior}, (1+\tau)\ell_{prior}], \\
    h &\in [(1-\tau)h_{prior}, (1+\tau)h_{prior}],
\end{aligned}
\end{equation}
where $\tau$ represents the error margin. $w_{prior}$, $l_{prior}$ and $h_{prior}$ are from LLMs-derived priors. This process results in an object bank $O = \{(b_i^{3D}, P_i)\}_{i=0}^{N_o}$, where $b_i^{3D}$ is the reserved box, $P_i$ comprises the LiDAR points within each box and $N_o$ is the total number of reserved boxes. 

For the current frame, we randomly select boxes from bank $O$ and integrate them at varying distances from the ego vehicle, ensuring diverse spatial distribution. The LiDAR points within each box are sampled according to their distance, with the sampling ratio defined as:
\begin{equation}
\label{equ: place object}
    r_{sampling} = \min(1, \frac{d-d_{new}}{d-d_{ori}}),
\end{equation}
where $d$ denotes the total range in the point cloud, $d_{ori}$ is the original distance of the object, $d_{new}$ is the distance post-placement. The selected boxes are denoted as $\mathcal{B}^t_{\rm spatial}$ and the collective set of boxes in the current frame is represented as $\mathcal{B}^t_{\rm final} =\mathcal{B}^t \bigcup \mathcal{B}^t_{\rm temporal} \bigcup \mathcal{B}^t_{\rm spatial}$.
This strategy aims to substantially enhance the visibility of generic objects in LiDAR data and the perception ability of the obtained model.

%particularly improving the detection of objects located at farther distances from the sensor.

%With this strategy, we are likely to increase the visibility of generic objects, improving the ability to perceive those located further from the sensor.

%To supervise distant objects effectively, we establish a minimal distance threshold. The above placement of objects are operated in distance greater than the threshold.
\noindent \textbf{Loss for Generic Object Perception.} With the obtained 3D boxes $\mathcal{B}^t_{\rm final} = \{b_{k}^{3D}\}_{k=1}^{V_{final}}$, we formulate the loss for generic object concept acquisition and localization. Utilizing a DETR-like structure, we extract features from LiDAR points and apply bipartite matching to determine the optimal permutation $\hat{\sigma}$, the loss is thus expressed as:
\begin{equation}
\vspace{-1em}
    \mathcal{L} = \sum_{k=1}^{N}[ \mathcal{L}_{\rm focal}(s_{\hat{\sigma}_i(k)}) + \mathcal{L}_{\rm L_1}(b_{\hat{\sigma}_i(k)}, b^{3D}_{k})],
\end{equation}
where $s_{\hat{\sigma}_i(k)}$ denotes whether it is an object or not, $\hat{\sigma}_i(k)$ is the element in $\hat{\sigma}$. $\mathcal{L}_{\rm focal}$ constrains the level of ``objectness'' of generated 3D boxes, $\mathcal{L}_{\rm box}$ considers the constraint on boxes. With this composite loss optimized, we obtain a model with the ability to perceive generic objects.

% in original DETR, we define the cost function to . The cost is expressed as:
% \begin{equation}
%     \hat{\sigma}_i = \argmin_{\sigma \in \mathfrak{S}_{N}}\sum_{k=1}^{N} [\mathcal{L}_{\rm binary}(s_{\sigma(k)}) + \mathcal{L}_{\rm box}(\hat{b}_{\sigma(k)}, \hat{b}^{3D}_{k})],
% \end{equation}
% where $s_{\sigma(k)}$ is the degree of ``objectness'' and $\hat{b}_{\sigma(k)}$ is the box prediction. The classification head becomes a binary classification problem, indicating it is object or not. When the optimal permutation $\hat{\sigma}_{i}$ is obtained in the $i$-th LiDAR point cloud,  %We consider all LiDAR training data together and can get the object-attention loss $\mathcal{L}_{\rm{object}} =\sum_{i=1}^{|\mathcal{D}|}\mathcal{L}_i$.

\subsection{Specific Semantics Interpretation}
\label{subsection: specific semantics interpretation}
To interpret the specific semantics of detected generic objects in LiDAR, we correlate objects across both LiDAR and image domains. We apply the model after generic object perception to a given LiDAR frame, producing boxes $\{b_i^{3D}\}_{i=0}^N$ and their corresponding features $\{f_i^{3D}\}_{i=0}^N$. Instead of using the image-level LVLs, \emph{e.g.}, CLIP, we opt for object-level LVLs, such as grounding DINO, which provides 2D boxes $\{b_{i=0}^{2D}\}_{i=0}^{N_{2D}}$, 2D object features $\{f_i^{2D}\}_{i=0}^{N_{2D}}$ and text embeddings $\{t_i\}_{i=0}^{N_{2D}}$ simultaneously.

For each detected 3D box $b_i^{3D}$, we project it to each view image with the corresponding intrinsic matrix $K_j$ and extrinsic matrix $E_j$, formulated as:
\begin{equation}
    \hat{b}_{ij}^{2D} = \textbf{K}_j \cdot \textbf{E}_j \cdot b_i^{3D}, \  j=1,...,m
\end{equation}
The $\hat{b}_{ij}^{2D}$ is further filtered and only those lying in the image are reserved.
For the reserved box $\hat{b}_{ij}^{2D}$, we compute the IoU with the 2D boxes $\{b_i^{2D}\}_{i=0}^{N_{2D}}$ from grounding DINO and find the most close one $b_j^{2D}$. The corresponding text embeddings $t_j^{2D}$ feature is retrieved. We then try to minimize the discrepancy between $f_i^{3D}$ and all 2D features that has the same text embeddings $t_j^{2D}$. Mathematically, it is expressed as: 
\begin{equation}
    \ell_{align} = -\frac{1}{N} \sum_{i=1}^{N} \log \frac{\sum_{j=0}^{N_i}e^{f_i^{3D} \cdot f_j^{2D}/ \delta}}{\sum_{k=0}^{N^{2D}} e^{f_i^{3D} \cdot f_k^{2D} / \delta}},
\end{equation}
where $N_i$ denote all 2D features that has the same text embeddings $t_j^{2D}$ for $b_i^{3D}$. Once the object-level alignment is finished, we can directly perform open-vocabulary LiDAR detection with the LiDAR input.

\noindent \textbf{2D-3D Integration.}
Considering that paired RGB images with LiDAR are always available in autonomous driving, we thus can perform 2D-3D feature integration. For each detected object, we have optimized 3D features $f_i^{3D}$ and identified the best matched 2D boxes feature $f_i^{2D}$, the similarity between 3D-2D features with the text embeddings in $\{t_i\}_{i=0}^{N_{2D}}$ are computed as follows:
\begin{equation}
\begin{aligned}
    s_j^{3D} &= \cos(f_i^{3D}, t_j), \\
    s_j^{2D} &= \cos(f_i^{2D}, t_j), \ j=0,...,N^{2D}
\end{aligned}
\end{equation}
We obtain the maximum value for 2D feature and 3D feature by $s^{3D} = \max_{j}\{s_j^{3D}\}_{j=0}^{N_{2D}}$,  $s^{2D} = \max_{j}\{s_j^{2D}\}_{j=0}^{N_{2D}}$, along with their semantic labels $c^{3D}$ and $c^{2D}$. The final label for object $i$ is determined by comparing $s_i^{2D}$ and $s_i^{3D}$, selecting the label associated with the larger value.

\noindent \textbf{Large Language Model (LLMs) Post-processing.}
The size priors from LLMs can be used to assist in recalibrating predictions. By matching the 3D IoU of predicted boxes with these size priors, we can determine the most matching prior and the corresponding sematic label. We then incorporate the predictions from size prior with results from 2D-3D integration by selecting label with the highest similarity.

% to determine the most accurate size. Since each size prior is associated with a semantic label, we can assign labels based on this correlation.

\subsection{Inference}
we first extract 3D object features from the LiDAR point cloud and align them with text embeddings from novel categories. LLMs post-processing is also applied in assisting in the determination of the final labels. Additionally, when RGB images are available, we enhance our detection process by integrating 3D and 2D features, thereby improving the accuracy of our semantic label determination.
 

%For simplicity, we actually use the detected 2D bounding boxes of grounding DINO in 3D boxes estimation. As indicated in Section~\ref{}, it can directly provides spatial location $\{b_i^{2D}\}$ and semantic. 

%For novel class detection, we first replace the class name ``Others'' with a specific class name, for example, "motorcycle" to generate the semantically-aware bounding boxes. We also input the class name and accompanying images into grounding DINO to get the 2D bounding boxes. To select the corresponding 3D boxes, we project the generated 3D bounding boxes into images and select the boxes with the highest IoU. It is worth noting that the selection process for novel classes could be slightly different from known classes. This kind of strategy is consistent with the training process and is found to be efficient.

%to alleviate the overfitting problem above. It concerns localizing the novel objects and designing the training loss for optimization. 

%Similar to known classes, we extract the text embedding for "Others" to obtain semantically-conditioned object queries.

















% \subsection{Closed-set DETR-based Model in LiDAR}
% \label{subsection: Closed-set DETR-based model in LiDA}
% Object detection task has seen a revolutionary shift from a surrogated problem reliant on proposals or anchors to a direct set prediction problem, with the development of DETR-based structure~\cite{carion2020end}. This advanced framework not only streamlines the overall pipeline but also substantially enhances detection efficiency. In the context of a closed-set DETR-based LiDAR detection model, the architecture mainly comprises a backbone, a transformer decoder, and feed-forward networks (FFNs). Specifically, the model first extracts LiDAR features from the backbone, which serve as key and value for the transformer decoder. Subsequently, it initializes $N$ learnable object queries for decoding. Based on the output of the transformer decoder, FFNs try to predict a set of $N$ predictions $\{\hat{y}_k\}_{k=1}^N = \{(\hat{b}_k, \hat{p}_k \in R^{C})\}_{k=1}^N$, where $\hat{b}_k$ refers to the predicted 3D bounding boxes and $\hat{p}_k$ denotes the predicted probability spanned in the label space $R^{C}$. To ensure all objects within the LiDAR data are captured, $N$ is consistently assumed to be larger than the actual number of target objects, $K$.

% %The backbone could be voxel-based, as proposed in~\cite{zhou2018voxelnet, yan2018second}. The decoder, typically similar to the structure in ~\cite{misra2021end}, consists of $L$ layers.
% %Object queries and LiDAR features interact with each other in the transformer decoder. 

% The training pipeline of the model involves two primary stages: optimal bipartite matching for paired indexes and loss computation based on paired results. Specifically, the model tries to establish a one-to-one mapping from predictions $\{\hat{y}_k\}_{k=1}^N$ to the ground truth $\{y_k \}_{k=1}^K$ in optimal bipartite matching. To achieve this, $\{y_k\}_{k=1}^K$ is first padded with $\varnothing$ (no object) to match with $N$, and then search for a permutation of $N$ elements, denoted as $\sigma \in \mathfrak{S}_N$, that yields the lowest matching cost:
% \begin{equation}
%     \hat{\sigma} = \argmin_{\sigma \in \mathfrak{S}_N} \mathcal{L}_{\rm cost}(\sigma) = \argmin_{\sigma \in \mathfrak{S}_N} \sum_{k=1}^N \big [\mathcal{L}_{\rm cls}(p_{\sigma(k)}) + \mathbbm{1}_{\{c_i \ne \varnothing\}}\mathcal{L}_{\rm box}(b_k, \hat{b}_{\sigma(k)}) \big ]
%     \label{equ: Hungarian cost},
% \end{equation}
% where $c_i$ is the label of $i$-th box, $\mathbbm{1}$ is an indicator function that equals to 1 if $c_i \ne \varnothing$ else 0. $\sigma(k)$ is the index in predicted boxes which matches with $k$ in ground truth bxoes. Intuitively, matching cost $\mathcal{L}_{\rm cost}(\sigma)$ considers both the error in semantic label assignment and the difference between predicted and ground truth boxes.

% The Hungarian algorithm~\cite{stewart2016end} can be used to efficiently optimize Eqn.~\eqref{equ: Hungarian cost} to find the optimal one-to-one mapping $\hat{\sigma}$. With obtained $\hat{\sigma}$, we compute the optimization loss on all matched pairs. Typically, focal loss~\cite{lin2017focal} is utilized for boxes classification and $L_1$ loss is employed for bounding box regression in the Bird's Eye View (BEV) space. The overall loss is then formulated as:
% \begin{equation}
%     \mathcal{L}_{\rm training} = \sum_{k=1}^N \big [\mathcal{L}_{\rm focal}(p_{\hat{\sigma}(k)}) + \mathbbm{1}_{\{c_i \ne \varnothing\}} \mathcal{L}_{L_1}(b_k, \hat{b}_{\hat{\sigma}(k)})\big ].
%     \label{equ: Hungarian loss}
% \end{equation}

% Given the unavailability of large-scale LiDAR-based datasets in our scenario, the strategy of pretraining~\cite{radford2021learning, liu2023grounding} to attain open-vocabulary capabilities is thus unfeasible here. Alternatively, we turn to the readily available 2D open-vocabulary detection models, for example, grounding DINO~\cite{liu2023grounding}. The idea is driven by two primary considerations: the accessibility of these models and the beneficial alignment of the text embedding with 2D visual concepts, assured by the pretraining on extensive detection and grounding datasets. As highlighted in the introduction, directly aligning known LiDAR objects with text embeddings extracted from 2D open-vocabulary models leads to an over-fitting problem. Given a novel class, the model tends to predict boxes on known objects.
% \subsection{LiDAR-Based Open-Vocabulary Framework}
% In this part, we establish our framework for open-vocabulary object detection, basically based on the DETR-based structure above. The framework consists of two parts: potential 3D bounding boxes generation for novel classes and object-centric loss for optimization.  

% \subsubsection{3D Bounding Boxes Generation}
% \label{subsection: Semantically-Conditioned Object Query}
% %Specifically, for given category $c_k$ in a LiDAR-based dataset, we employ the text encoder $\mathcal{T}_{\rm DINO}$ in grounding DINO to generate the corresponding text embedding $z_k^{text} = \mathcal{T}_{\rm DINO}(c_{k})$. Theoretically, the extracted text embedding $z_k^{text}$ is tailored to identify the corresponding objects in 2D images. To transfer the alignment ability to LiDAR-based data, we try to associate the paired LiDAR features $f$ with the generated text embeddings $z_k^{text}$, based on the known classes in the training set. This process is expected to facilitate the generalization of alignment capabilities to novel classes. In other words, given a class without direct association, the generated text embedding is still expected to detect the corresponding objects in LiDAR space.
% To localize the novel objects, we consider all potential objects across classes and introduce an additional semantic label, ``Others''. It is denoted as $c_{o}$. This label is intended to denote all unknown objects besides objects with ground truth, without being confined to a specific class.

% Specifically, given $c_o$, we employ the text encoder $\mathcal{T}_{\rm DINO}$ in grounding DINO to generate the corresponding text embedding $z_o^{text} = \mathcal{T}_{\rm DINO}(c_{o})$. We then condition original object queries on the text embedding $z_o^{text}$. %Initially, we update original semantically-agnostic object queries by incorporating the extracted semantically-aware embedding $z_k^{text}$. 
% Mathematically, such an operation can be expressed as:
% \begin{equation}
%     q{'} = q \oplus f_{\rm proj}(z_o^{text}), 
% \end{equation}
% where $\oplus$ denotes the operation of addition and $f_{\rm proj}$ represents the introduced fully-connected layer to ensure dimensional compatibility between $z_o^{text}$ and the original query $q$. We term the updated object queries $q{'}$ as semantically-conditioned object queries.

% Next, with the category information encoded into the queries $q{'}$, we feed them into the transformer decoder to interact with extracted LiDAR feature from the backbone. It is then processed by FFNs to obtain a set of semantically-aware 3D bounding boxes $\hat{Y}_{others}^{3D} = \{\hat{b}_k\}_{k=1}^N$.

% %Theoretically, the extracted text embedding $z_o^{text}$ is tailored to identify the corresponding objects in 2D images. To transfer the alignment ability to LiDAR-based data, we try to associate LiDAR features $f$ with text embeddings $z_o^{text}$ on the known classes. It is expected that a novel class with extracted embedding could associate with its corresponding objects in LiDAR.

% %This process is expected to facilitate the generalization of alignment capabilities to novel classes. In other words, given a class without direct association, the generated text embedding is still expected to detect the corresponding objects in LiDAR space.

% %A straightforward method to achieve the association between $f$ and $z_k^{text}$ is
% Our framework naturally adapts to known classes since they all possess the ground truth semantic label. We can directly extract text embeddings for these labels and condition original object queries on each of them. Our framework can thus generate 3D box candidates for both known classes and novel classes simultaneously, which largely streamlines the process of 3D box generation.

% %Next, with the category information encoded into the queries $q{'}$, we eliminate the requirement of predicting the semantic label of 3D boxes in the fixed label space $R^C$. We just need to output a score $s_k$ to indicate whether $k$-th box matches with the input queries. We realize this by replacing the original classification head with a binary classifier. In optimization, we basically follow the above structure but replace the $\hat{p}_k$ with $s_k$ in matching cost $L_{\rm cost}(\sigma)$ to obtain $\hat{\sigma}$. Finally, we get the updated training loss as:
% % \begin{equation}
% %     \mathcal{L}_{\rm training} = \sum_{k=1}^N \big [\mathcal{L}_{\rm focal}(s_{\hat{\sigma}(k)}) + \mathbbm{1}_{\{c_i \ne \varnothing\}} \mathcal{L}_{L_1}(b_k, \hat{b}_{\hat{\sigma}(k)})\big ].
% %     \label{equ: updated Hungarian loss}
% % \end{equation}


% %The cost for  and training loss for optimization are then updated accordingly. Given the matching score $\hat{s}_k$ from the binary classifier and 3D bounding boxes $\hat{b}_k$. The cost for optimal bipartite matching becomes:
% %\begin{equation}
% %   \hat{\sigma} = \argmin_{\sigma \in \mathfrak{S}_N} \sum_{i=1}^N \big [\mathcal{L}_{\rm match}(s_k) + \mathbbm{1}_{\{c_k \ne 0\}} \mathcal{L}_{\rm box}(b_k, \hat{b}_{\sigma(k)}) \big ] \label{equ: updated Hungarian cost.}
% %\end{equation}
% %Compared with Eqn.~\eqref{equ: Hungarian cost}, the $\mathcal{L}_{\rm cls}(p_{\sigma(k)})$ cost is replaced with $\mathcal{L}_{\rm match}(s_k)$ in Eqn.~\eqref{equ: updated Hungarian cost.}. We use the same Hungarian algorithm to obtain the optimal permutation $\hat{\sigma}$ in matching. For optimization, we adopt the same loss as in Eqn.~(\eqref{equ: Hungarian loss}) but only replace the original probability $p_{\hat{\sigma}(k)}$ with $s_{\hat{\sigma}(k)}$ in focal loss $\mathcal{L}_{\rm focal}(\cdot)$.

% %These modifications make the model feasible to perform open-vocabulary tasks. Given a new category of interest, the model can simultaneously take the category name and LiDAR data as input, producing the corresponding 3D bounding boxes. However, To address this issue, we consider more advanced 2D-3D modeling and constrain on the objects of novel classes.

% %the above loss primarily involves the supervision of known classes with ground truth. For novel classes, there is no explicit constraint on the objects.

% %The semantically-conditioned queries $q{'}$ interact with the LiDAR features in the transformer decoder. After that, the FFNs decode the corresponding matching score wi

% %The utilization of semantic labels is a key component in both bipartite matching and loss computation in the model above. However, it is worth noting that these labels are typically produced within the confined $R^C$ space. Thus, directly adopting the structure above is not feasible for open-vocabulary object detection, where the semantic labels are theoretically expanded in $R^{\infty}$. To overcome this challenge and enable the conventional closed-set architecture to perform open-vocabulary detection, we first remove the class prediction head and try we resort to  and condition the original object queries on the semantic embeddings extracted from 2D pretrained model.

% \subsubsection{Object-Centric Loss}
% However, even with the generate 3D boxes, imposing extra constraints on novel classes in LiDAR data is not trivial. The generated 3D boxes for novel classes actually lack ground truth for supervision. To resolve this, we leverage the image encoder $\mathcal{I}_{\rm DINO}$ of grounding DINO to generate 2D bounding boxes for supervision. Even though grounding DINO is an open vocabulary with large visual concepts, directly localizing objects in an image with the class name "Others" is challenging, due to its broad meaning. In practice, we concretize the concept of ``Others'' with common classes found in autonomous driving scenarios, such as "people, columns, manhole cover," and use these surrogated classes to generate 2D bounding boxes. Take one LiDAR frame as example, there are $m$ accompanied images $\{I_j\}_{j=1}^{m}$ collected in different views. For each image, we could obtain the bounding boxes $(b_{jk})_{k=1}^{V_j}$, where $V_j$ denotes the number of 2D objects detected in $j$-th view. Considering all views together, we get all the detected boxes $\{(b_{jk}^{2D})_{k=1}^{V_j}\}_{j=1}^{m}$. We emphasize that the selected categories to concretize the concept of ``Others'' is not that important as long as it is meaningful, since our primary goal is to identify missed objects besides those in the known class.

% Given the predicted 3D bounding boxes $\hat{Y}_{\rm others}^{3D}$ for ``Others'', we project each 3D boxes $\hat{b}_k$ in $\hat{Y}_{\rm others}^{3D}$ into each image view. For simplicity, we illustrate this process using the $j$-th view as an example. Mathematically, this can be represented as:
% \begin{equation}
%     \hat{b}_{jk}^{2D} = \textbf{K}_j \cdot \textbf{E}_j \cdot \hat{b}_k, 
% \end{equation}
% where $\textbf{K}_j$ and $\textbf{E}_j$ are intrinsic and extrinsic matrix, respectively. In practice, the projected boxes may fall outside the image. In that case, we discard those boxes and reserve those within the image. Thus, the number of boxes $V_j$ after projection is smaller than the original number $N$. 

% Based on the projected 2D boxes $(\hat{b}_{jk}^{2D})_{k=1}^{V_j}$ in $j$-th view and the generated 2D bounding boxes $(b_{jk}^{2D})_{k=1}^{V_j}$ from grounding DINO, we construct the object-centric loss to constrain objects of novel classes. Similar to the operation in section~\ref{subsection: Closed-set DETR-based model in LiDA}, we need to determine the optimal permutation $\hat{\sigma}_j$ in bipartite matching to calculate the final loss. The cost is defined as:
% \begin{equation}
%     \hat{\sigma}_j = \argmin_{\sigma \in \mathfrak{S}_{V_j}}\sum_{k=1}^{V_j} \mathcal{L}_{\rm box}(b_{jk}^{2D}, \hat{b}^{2D}_{j\sigma(k)}),
% \end{equation}
% where we only rely on the cost of boxes and ignore the cost of label assignment. The reason is that the cost of label assignment works little in practice for our purpose of avoiding box overfitting and generating more accurate boxes. When the optimal permutation $\hat{\sigma}_{j}$ is obtained in the $j$-th view, the object-centric loss on paired 2D bounding boxes can be expressed as:
% \begin{equation}
%     \mathcal{L}_j = \sum_{k=1}^{V_j} \mathcal{L}_{\rm box}(b_{jk}^{2D}, \hat{b}^{2D}_{j\hat{\sigma}_j}),
% \end{equation}
% where $\mathcal{L}_{\rm box}$ actually considers both $L_1$ loss on box coordinates and IoU loss on the overlaps. Further, we consider all views together and can get the object-centric loss $\mathcal{L}_{\rm{object}} =\sum_{j=1}^{m}\sum_{k=1}^{V_j}\mathcal{L}_{\rm box}(\hat{b}^{2D}_{j\hat{\sigma}_j}, b_{jk}^{2D})$.

==> sec/4_experiments.tex <==
\section{Experiments}
%In this section, we elaborate on our experimental settings and analyze the performance of OpenSight, highlighting the effectiveness and generalization ability of the proposed framework.
\subsection{Experimental settings}
\label{sec: experimental settings}
\noindent \textbf{Dataset.}
We conduct our open-vocabulary experiments on nuScenes~\cite{nuscenes} dataset, a large-scale, outdoor dataset featuring multimodal data modalities. Each frame in the dataset contains data from one 32-beam LiDAR and six cameras, offering a comprehensive view of the surroundings. The dataset comprises 1000 scenes in total, with up to 1.4 million annotated 3D bounding boxes spanning 10 classes. We reserve all the classes as novel to evaluate the effectiveness of our proposed OpenSight. 
%In order to evaluate the effectiveness of our proposed OpenSight, we partition the dataset into known and novel classes, with 8 of the 10 classes designated as known, and the remaining 2 classes as novel (``motorcycle'' and ``pedestrian''). 
%For quantitative evaluation, we employ the nuScenes Detection Score (NDS) and mean Average Precision (mAP) metrics on both known classes and novel classes, following the official nuscenes-devkit.

\noindent \textbf{Evaluation Metrics.}
For quantitative evaluation, we initially employ Average Precision (AP) on each class and mean Average Precision (mAP) across all novel classes. Considering LiDAR point density variation with distance, we introduce distance-based mAP metrics: mAP-near, mAP-midrange, and mAP-far. Similarly, acknowledging the size disparities among objects in different classes (e.g., `bus' vs. `traffic\_cone'), we categorize classes into `large', `medium', and `small' and propose mAP-large, mAP-medium, and mAP-small. More details are in the Appendix.

\noindent \textbf{Implementation.}
We use VoxelNet~\cite{zhou2018voxelnet} as our LiDAR backbone and voxelize the LiDAR point cloud by the default settings in~\cite{yin2021center, bai2022transfusion}. For designed novel classes, we eliminate the usage of ground truth labels in training. We use the ``bert-base-uncased'' encoder in grounding DINO for text embedding extraction. %For better expression ability, we also apply similar prompt templates as CLIP~\cite{radford2021learning}. 
%To generate pseudo-GT for the supervision of novel classes, 
For convenience, we also apply grounding DINO to extract 2D boxes. The accompanying images with a high resolution of 900 $\times$ 1600 are directly fed into grounding DINO for accurate 2D box generation and corresponding object-level features generation. The number of object queries is set to 200. We adopt the AdamW optimizer and jointly optimize the 3D loss in known classes and the 2D loss in novel classes for 20 epochs. The learning rate and weight decay are set as 1.0e-4 and 0.01, respectively. The code is implemented in PyTorch with the open-sourced MMDetection3D~\cite{mmdet3d2020}.
\begin{table*}[t]
\footnotesize
  \centering
  \setlength{\tabcolsep}{6pt}
  \begin{tabular}{l|cc|cccccccccc}
    \toprule
    Method   & mAP & NDS &\scriptsize Car &\scriptsize Truck &\scriptsize C.V. &\scriptsize Bus &\scriptsize Trailer &\scriptsize Barrier &\scriptsize Bicycle &\scriptsize Traffic\_cone &\scriptsize Motorcycle  &\scriptsize Pedestrian\\
    \midrule
    Supervised~(box+label) & 57.3 &61.7 & 86.0 & 38.8 & 18.3 & 63.3 & 34.2 &70.5 &46.7 &70.2 &59.5 &85.2\\
    Supervised~(box only) & 34.2 &39.0 & 53.2 & 20.1 & 7.4 & 20.5 & 0.7 &50.1 &37.8 &52.6 &39.1 &60.8\\
    \midrule
    Detic-3D~\cite{zhou2022detecting} &5.8 &12.7 &15.1 &2.9 & 2.1 & 4.2 &0.0 & 0.1 & 6.2 & 0.8 & 6.1 & 21.1\\
    OWL-ViT-3D~\cite{minderer2022simple} &5.4 &12.4 &14.2 &2.5 & 1.8 & 4.0 &0.0 & 0.1 & 5.2 & 1.1 & 5.5 & 19.4\\
    \midrule
    OV-PointCLIP~\cite{zhang2022pointclip} &0.1 &5.0 &0.0 &0.0 &0.0 &0.0 &0.0 &0.0 &0.7 &0.2 &0.0 &0.1 \\
    OV-PointCLIPv2~\cite{Zhu2022PointCLIPV2} &2.8 &10.9 &0.0 &2.7 &0.0 &0.0 &0.0 &22.0 &0.0 &0.2 &0.0 &3.2\\
    CLIP-3D~\cite{radford2021learning} &7.2 &14.2 & 9.6 & 2.8 & 2.1 &2.6 &0.0 & 0.1 &11.5 & 14.4 &9.8 & 18.9\\
    OV-3DET~\cite{lu2023open} &5.7 &12.0 &16.1 &2.9 &0.3 &1.3 &0.0 & 0.3 &1.8 &11.0 &2.0 &21.1\\
    CoDA~\cite{cao2023coda} &10.3 &16.1 &85.5 &1.9 &0.0 &2.0 &0.0 &0.0 &3.9 &0.0 & 5.9 &3.5 \\
    \midrule
    %OV-Transfusion~\cite{bai2022transfusion} & 47.1 & 84.0 & 51.5 & 22.5 & 68.4 & 48.3 & 69.7 & 49.2 & 75.5 & 1.9 & 1.0\\
    %OV-BEVFusion~\cite{liang2022bevfusion} & 47.6 & 86.9 & 51.3 & 26.0 & 70.2 & 46.2 & 67.1&50.5 & 75.1 & 2.0 & 1.7\\
    %\midrule
    %Proj-PointPillar~\cite{lang2019pointpillars}& 21.1 & 68.0 & 22.1 & 3.9 & 27.3 & 22.5 & 37.6 & 1.0 &27.3 & 1.0 &1.2 \\
    %Proj-CenterPoint~\cite{yin2021center} & 43.1 & 82.5 & 50.9 & 19.0 & 58.8& 39.3 & 67.2 & 39.0 & 69.2& 3.0 & 3.1     \\
    %Proj-MVP~\cite{yin2021multimodal}  & 45.9 & 54.3 &85.3 & 23.5 & 59.0& 53.5 & 67.8 & 42.3 & 68.7 &3.9 & 3.4 \\
    %SAM-3D~\cite{kirillov2023segany}  & 46.4 &84.5 &50.3 & 23.0 & 67.9 & 47.6 & 68.8 &47.2 & 73.0 & 2.5 & 2.2  \\
    OpenSight~(Ours) & 23.5 &24.0 & 32.1 & 11.6& 8.7 & 5.1 & 0.8 & 42.2 & 26.1 & 25.6 & 30.4 & 52.5\\
    \bottomrule
  \end{tabular}
  \vspace{-1em}
  \caption{Results on NuScenes dataset. All classes are reserved as novel classes. AP of each class and mAP across all classes are shown. ``Car'' in CoDA is the known class and is fully supervised. (`C.V' is denoted as `construction\_vehicle' here.)}
  \label{tab: overall results}
  \vspace{-1em}
\end{table*}
\subsection{Baselines}
As there are no direct baselines addressing open-vocabulary LiDAR-based 3D detection, we primarily construct the baselines based on well-known works~\cite{zhou2022detecting, Zhu2022PointCLIPV2, radford2021learning, cao2023coda, lu2023open} 
and compare with OpenSight. Specifically, they are:

\noindent \textbf{Fully-supervised training.} Initially, we perform fully supervised training across all categories, establishing an upper bound for the open-vocabulary detection performance. We consider using both ground-truth boxes and labels (`Supervised~(box+label)') or just using ground-truth boxes (`Supervised~(box only)'). 

%\paragraph{Closed-set methods.} In this part, we select three representative LiDAR-based detectors CenterPoint~\cite{yin2021center}, Transfusion~\cite{bai2022transfusion}, and BEVFusion~\cite{liang2022bevfusion}, as our baselines. To validate open-vocabulary performance, we maintain the original label space in the classifier while excluding the training data of novel classes. This strategy allows us to assess the ability of the selected baselines to generalize to unseen categories.

\noindent \textbf{2D open-vocabulary methods.} Detic~\cite{zhou2022detecting} is a pioneer work in the realm of 2D open-vocabulary object detection tasks and can detect 21K classes. It is thus desirable for our study here. OWL-ViT~\cite{minderer2022simple} decodes the object labels and boxes directly from the pre-trained features and shows good robustness in real-world applications. With the 2D detection results of either Detic or OWL-ViT, we adopt the same procedure in Section~\ref{subsection: generic object perception} to obtain the corresponding 3D bounding boxes in LiDAR space. These two baselines are denoted as Detic-3D and OWL-ViT-3D.
% provides a streamlined framework for open-vocabulary detection. It

\begin{table}
\footnotesize
  \centering
  \begin{tabular}{l|ccc}
    \toprule
    Method & mAP-near & mAP-midrange &mAP-far\\
    \midrule
    Detic-3D~\cite{zhou2022detecting} &18.5 &9.3 & 5.8 \\
    OWL-ViT-3D~\cite{minderer2022simple} &17.3 &8.2 &5.4\\
    OV-PointCLIP~\cite{zhang2022pointclip} &0.2 &0.1 &0.1 \\
    OV-PointCLIPv2~\cite{Zhu2022PointCLIPV2} &4.5 &3.6 &2.8 \\
    CLIP-3D~\cite{radford2021learning} &18.8 &11.2 &7.2\\
    OV-3DET~\cite{lu2023open} &16.1 &9.9 &5.7\\
    CoDA~\cite{cao2023coda} &18.2 &16.6 &10.3\\
    OpenSight (Ours) &28.0 &26.5 & 23.5\\
    \bottomrule
  \end{tabular}
  \vspace{-1em}
  \caption{Performance \emph{w.r.t} mAP-near, mAP-medium, mAP-far.}
   \label{tab: evaluation of distance}
  \vspace{-1em}
\end{table}
\noindent \textbf{3D open-vocabulary methods.} We then consider the latest open-vocabulary point cloud classification methods and a variety of indoor open-vocabulary works to evaluate their performance in our tasks here. Specifically, we utilize a fully-supervised method to generate pseudo boxes and employ PointCLIP~\cite{zhang2022pointclip}, PointCLIPv2~\cite{Zhu2022PointCLIPV2}, denoted as ``OV-PointCLIP'', ``OV-PointCLIPv2''. We also combine our predicted boxes and CLIP~\cite{radford2021learning} for this task (``CLIP-3D''). Meanwhile, we adapt the latest works OV-3DET~\cite{lu2023open} and CoDA~\cite{cao2023coda} in indoor settings to our task here and demonstrate the effectiveness of our proposed methods. 

%\paragraph{Outdoor open-vocabulary methods.} Currently, there are very limited open-vocabulary works in autonomous driving due to the complexity of real-world settings and the large gap between existing 2D open-vocabulary models. We adapt the existing supervised methods, \emph{e.g.}, to our setting. For object localization, we adopt xx~\cite{} for xx.

%\paragraph{Projected methods.} We also consider generalizing a set of closed-set models for detecting novel classes by leveraging the large-scale 2D open-vocabulary models, such as ground DINO~\cite{liu2023grounding}. Initially, we project the generated 3D boxes into 2D images, then we compute the overlaps between projected 2D boxes and those inferred by 2D open-vocabulary models to perform box selection and label assignment. This approach facilitates the transformation of various closed-set methods into open-vocabulary models. We conduct the experiments on PointPillar~\cite{lang2019pointpillars}, CenterPoint~\cite{yin2021center}, MVP~\cite{yin2021multimodal} and term them as Proj-PointPillar, Proj-CenterPoint, and Proj-MVP, respectively. Furthermore, we can utilize SAM~\cite{kirillov2023segany} for detecting objects in novel classes. Initially, we apply SAM to generate a collection of 2D masks. Then, point clouds are projected into the image plane and only those within the masks are selected. Finally, we compute the minimum enclosing bounding box for the selected point clouds to get the predicted boxes.

\begin{table}
\footnotesize
  \centering
  \begin{tabular}{l|ccc}
    \toprule
    Method & mAP-large &mAP-medium &mAP-small\\
    \midrule
    Detic-3D~\cite{zhou2022detecting} &5.3 &4.1 & 11.0\\
    OWL-ViT-3D~\cite{minderer2022simple} &4.9 &3.7 &10.3\\
    OV-PointCLIP~\cite{zhang2022pointclip} &0.0 &0.3 & 0.2\\
    OV-PointCLIPv2~\cite{Zhu2022PointCLIPV2} &0.6 &7.3 &1.6\\
    CLIP-3D~\cite{radford2021learning} &3.4 &7.1 & 16.7 \\
    OV-3DET~\cite{lu2023open} &4.1 &1.4 &16.0 \\
    CoDA~\cite{cao2023coda} &17.9 &4.9 &1.8 \\
    OpenSight (Ours) &11.5 &32.9 & 39.0\\
    \bottomrule
  \end{tabular}
    \vspace{-1em}
    \caption{Performance \emph{w.r.t} mAP-large, mAP-medium, mAP-small.}
  \label{tab: evaluation of object sizes}
  \vspace{-1em}
\end{table}

\subsection{Main results}
In this section, we discuss the performance of our model on novel classes, as summarized in Table~\ref{tab: overall results}. Despite the lack of 3D ground truth supervision, our framework demonstrates strong overall open-vocabulary ability across classes. Notably, it achieves exceptional performance in some classes, for example, 52.5 AP in `pedestrian' and 42.2 AP in `Barrier'. Unfortunately, we also notice the limited performance in `Trailer', with 0.8 AP. To analyze this, we compare with `Supervised~(box only)', where groundtruth boxes are used and only 0.7 AP is achieved in `Trailer', we thus attribute the reason to label alignment with grounding DINO rather than box inaccuracy. Grounding DINO offers limited help in fine-grained classes. Our model also shows superior performance when compared with the baselines.  Specifically, we observe that PointCLIP is very limited in detecting novel objects and CLIP-3D achieves the best overall performance with our detected boxes. CoDA, while effective in known classes like `car', falls short in novel class adaptation, averaging only 1.9\% accuracy across novel categories.

Our more detailed evaluations, using distance-based metrics and size-based metrics, are presented in Tables~\ref{tab: evaluation of distance} and~\ref{tab: evaluation of object sizes}, respectively. The evaluation in Table~\ref{tab: evaluation of distance} reveals a trend where detection accuracy is higher for objects closer to the sensor. This is attributed to their denser point clouds and more defined geometric features. Conversely, detection accuracy decreases with increasing distance, likely due to sparser data and less distinct object outlines. Regarding size-based performance (Table~\ref{tab: evaluation of object sizes}), our model shows superior results for medium and small-sized objects. Large objects present lower detection rates, mainly due to their incomplete LiDAR scans. Additionally, the fine-grained categorization of large vehicles, such as `Trailer' and `Construction\_vehicle', complicates their accurate detection.

%The performance across different methods basically follows this pattern: the more recent the method, the higher its performance.

\subsection{Qualitative results on novel classes}
As shown in Figure~\ref{fig: visualization of detection results.}, our framework demonstrates a strong ability to detect novel objects by inputting the interested categories. We visualize the results from both BEV and a specific perspective. For example, our method successfully identifies the `pedestrian', `barrier', and `traffic\_cone' in example (a), and the `car' and `motorcycle' in (c). These results also indicate that our method exhibits superior open-vocabulary detection ability across different scenes.

\begin{table}
\setlength{\tabcolsep}{4pt}
\footnotesize
  \centering
  \begin{tabular}{c|cc|ccc}
    \toprule
    \# & Temporal & Spatial &mAP-near &mAP-midrange &mAP-far\\
    \midrule
    (1) & & &27.1 &24.8 & 22.1  \\
    (2) &\checkmark & &27.4 &25.9 & 23.0\\
    (3) & &\checkmark &27.5 &26.0 & 22.8\\
    (4) &\checkmark &\checkmark &28.0 & 26.5 &23.5\\
    \bottomrule
  \end{tabular}
  \vspace{-1em}
  \caption{Results with temporal and spatial awareness \emph{w.r.t} mAP-near, mAP-medium, mAP-far.}
  \label{tab: component in generic object}
  \vspace{-1em}
\end{table}

\begin{figure*}[t]
  \centering  \includegraphics[width=0.85\textwidth]{images/example1.png}
  %\fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \vspace{-1em}
  \caption{Visualization of detected novel classes in different LiDAR frames. (a) Detected `barrier', `traffic\_cone', and `pedestrian'; (b) Detected `car' and `pedestrian'; (c) Detected `car' and `motorcycle'; (d) Detected `barrier' and `pedestrian'.}
  \label{fig: visualization of detection results.}
  \vspace{-1em}
\end{figure*}
\subsection{Ablation}
In this part, we present a comprehensive analysis of OpenSight and examine the effectiveness of each component.

\noindent \textbf{Components in Generic Object Perception.}
We decouple the components in generic object perception and record the results in Table~\ref{tab: component in generic object}. Specifically, both modules improve more for mAP-medium and mAP-far. For example, temporal improves 1.1 AP for mAP-medium while 0.3 AP for mAP-near. Both modules interact positively with each other and further improve the results when jointly introduced.
%Here, we study the components of the proposed framework and parameter $\lambda$ in optimization loss.

\noindent \textbf{Components in Semantic Interpretation.}
We analyze the modules of direct alignment, 3D-2D feature integration, and LLMs priors in semantic interpretation and record the results in Table~\ref{tab: component in semantic integration}.
The performance is consistently improved with integration and priors introduced. Compared with LLMs priors, 3D-2D integration brings more benefits, for example, 0.9 \emph{vs.} 0.2 in mAP-medium. 

\begin{table}
\setlength{\tabcolsep}{4pt}
\footnotesize
  \centering
  \begin{tabular}{c|ccc|ccc}
    \toprule
    \# & D.A &I.G. &Priors &mAP-large &mAP-medium &mAP-small \\
    \midrule
    (1) &\checkmark & & &9.4 &31.8 &38.1 \\ 
    (2) &\checkmark &\checkmark & &10.9 &32.7 &38.8 \\
    % (3) &\checkmark &\checkmark & &11.3 &32.5 &38.7 \\
    (3) &\checkmark &\checkmark &\checkmark &11.5 &32.9 &39.0\\
    \bottomrule
  \end{tabular}
   \vspace{-1em}
   \caption{Results with direct alignment (`D.A.'), 3D-2D feature integration (`I.G.'), and LLMs priors.}
  \label{tab: component in semantic integration}
  \vspace{-1em}
\end{table}

\noindent \textbf{Image-level \emph{vs.} Object-level.} 
We also investigate the image-level open-vocabulary model CLIP~\cite{radford2021learning} in semantic interpretation. The results are recorded in Table~\ref{tab: different LVLs}. Compared with our adopted object-level grounding DINO, we notice that object-level alignment shows much better results from either a distance perspective or a size perspective. For example, 28.0 AP of near objects is achieved in object-level alignment, 9 points higher than image-level alignment. We analyze that CLIP requires more accurate bounding box prediction, in comparison with object-level alignment which only requires a nearest box. 

\noindent \textbf{Importance of Bounding Boxes Existence.} 
Existing open-vocabulary methods focus more on the alignment between 3D features and 2D features. However, in LiDAR-based object detection, we emphasize that accurate bounding boxes are essential before alignment. We select some classes and investigate both average precision (AP) and average recall (AR) under different thresholds. The results are recorded in Table~\ref{tab: importance of boxes existence}. Compared with AP, we observe a higher recall value in different threshold, indicating that although we can recall the correct objects, more objects with incorrect sizes are also recalled. Such results motivate that if we can obtain a more precise estimation of objects, the results will be improved further.

\begin{table}
\setlength{\tabcolsep}{3.5pt}
\footnotesize
  \centering
  \begin{tabular}{l|ccc|ccc}
    \toprule
    mAP & -near & -midrange & -far &-large &-medium &-small \\
    \midrule
    CLIP &19.0 &11.9 &8.2 &3.9 &8.2 &18.4 \\ 
    \midrule
    \makecell{Grounding \\DINO} &28.0 &26.5 &23.5 &11.5 &32.9 &39.0\\
    \bottomrule
  \end{tabular}
   \vspace{-1em}
  \caption{Results of image-level and object-level models.}
  \label{tab: different LVLs}
  \vspace{-1em}
\end{table}

\begin{table}
\setlength{\tabcolsep}{4.7pt}
\footnotesize
  \centering
  \begin{tabular}{l|ccc|ccc}
    \toprule
    \#CLASS & AP-0.5 & AP-1 & AP-2 & AR-0.5 & AR-1 & AR-2\\
    \midrule
    Car &4.7 &18.3 &45.9 &40.0 &69.0 &84.4\\ 
    Truck &0.2 &3.0 &13.3 & 13.2 &30.0 &51.1\\
    Pedestrian &38.8 &51.6 &57.1 &58.4 &69.3 &74.2\\
    \bottomrule
  \end{tabular}
  \vspace{-1em}
  \caption{AP and AR of some classes under different threshold.}
  \label{tab: importance of boxes existence}
  \vspace{-1em}
\end{table}

% \begin{table}


% \begin{table}

==> sec/5_conclusion.tex <==
\section{Conclusion}
We present OpenSight, a simple and versatile open-vocabulary framework for LiDAR-Based object detection. In the absence of ground-truth boxes and semantic labels, OpenSight first learns to identify and localize a wide range of generic objects. To boost the ability of generic object perception, we incorporate temporal and spatial awareness techniques that recalibrate and improve the visibility of estimated 3D boxes. We also align LiDAR object features with the 2D features from the grounding DINO for semantic interpretation. The extensive experiments demonstrate the effectiveness and generalization ability of the proposed framework, paving the way for further exploration in LiDAR-based open-vocabulary challenges.

% We present OpenSight, a simple and generic open-vocabulary framework for LiDAR-Based object detection. Based on the DETR-like structure, our initial exploration reveals that directly aligning LiDAR features with 2D text embeddings on known classes results in an overfitting issue. We thus design a complementary object-centric loss on novel objects to regulate the detection performance, leveraging 3D outputs and 2D open-vocabulary models. The extensive experiments demonstrate the effectiveness and generalization ability of the proposed framework. We hope that our work will inspire further investigation of LiDAR-based open-vocabulary problems in autonomous driving.

%\paragraph{Broad Impacts Statement and Limitations.}
%This paper studies the LiDAR-based open-vocabulary object detection problem. The capacity of open perception is a fundamental requirement for the deployment of autonomous vehicles and ensuring the safety. Potentially, it endows the model with human-like generalization ability, hence it can identify unforeseen objects and make corresponding decisions. The open vocabulary ability also facilitates the mining of new data to involve more objects of interest in the training. At present, though OpenSight has achieved much progress in novel categories, the performance is still considerably inferior when compared to the results obtained through supervised learning. Thus, the model may pose safety threats when applied in practice. However, as the first attempt to study open vocabulary problems in a real-world scenario, this research may inspire subsequent studies in this area.
